Building Your Own Trusted Execution Environments Using FPGA

In recent years, we have witnessed unprecedented growth in using hardware-assisted Trusted Execution Environments (TEE) or enclaves to protect sensitive code and data on commodity devices thanks to new hardware security features, such as Intel SGX and Arm TrustZone. Even though the proprietary TEEs bring many benefits, they have been criticized for lack of transparency, vulnerabilities, and various restrictions. For example, existing TEEs only provide a static and fixed hardware Trusted Computing Base (TCB), which cannot be customized for different applications. Existing TEEs time-share a processor core with the Rich Execution Environment (REE), making execution less efficient and vulnerable to cache side-channel attacks. Moreover, TrustZone lacks hardware support for multiple TEEs, remote attestation, and memory encryption. In this paper, we present BYOTee (Build Your Own Trusted Execution Environments), which is an easy-to-use infrastructure for building multiple equally secure enclaves by utilizing commodity Field Programmable Gate Arrays (FPGA) devices. BYOTee creates enclaves with customized hardware TCBs, which include softcore CPUs, block RAMs, and peripheral connections, in FPGA on demand. Additionally, BYOTee provides mechanisms to attest the integrity of the customized enclaves' hardware and software stacks, including bitstream, firmware, and the Security-Sensitive Applications (SSA) along with their inputs and outputs to remote verifiers. We implement a BYOTee system for the Xilinx System-on-Chip (SoC) FPGA. The evaluations on the low-end Zynq-7000 system for four SSAs and 12 benchmark applications demonstrate the usage, security, effectiveness, and performance of the BYOTee framework.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> applications.tex <==
\section{\sysname Applications}

\subsection{Example Application: Secure Audio DRM}

Designing a secure audio DRM was a challenge in 2020 MITRE Collegiate Embedded Capture-The-Flag competition (eCTF).

==> apps.tex <==
\section{\sysname Applications}
\label{s:apps}
In this section, we use multiple security-sensitive application examples to demonstrate how \sysname can secure real-world applications in several classes, namely computational application, peripheral interacting application, and peripheral and PS interacting application.
We present the design of an example application in each class, which we use to evaluate \sysname.
%For each application, we describe their architectures  \sysname. 
%We evaluate the performance of the applications in terms of memory usage and bla bla.

%\subsection{BYOT FW Interfaces}
%The \firmware and the SSC applications are developed and compiled as a separate standalone applications.
%The \firmware responsible for loading and executing the SSC applications on at run-time.
%Additionally, the \firmware provides some interfaces to the SSC applications.
%For instance, the SSC application 
%Even though the SSCs are developed and compiled as separate applications, the \firmware needs to reserve memory spaces for the SSC code and data sections.
%Furthermore, the \firmware will act as a library at runtime.
%For these reasons, we provide the linker script to compile the SSC application that maintains those constraints.
%Besides using our provided linker script for compilation, the developers need to define the entry point function of their SSC applications.
%The FW will begin executing the SSC application from this developer-defined entry point function.
%\begin{lstlisting}[ label={header},caption={Header file defining SSC entry}, language=c] 
%#ifndef BYOT_HEADER_H_
%#define BYOT_HEADER_H_
%
%int main() __attribute__ ((section (".text.ssc_entry")));
%
%#endif
%\end{lstlisting}
%Listing~\ref{header} illustrates an example defining the \emph{main} function as the entry point of the application.

%\firmware provides interfaces for the PS application to execute the SSCs on the CTEEs.
%i) \textit{LdExec} interface with the SSC name as an argument, loads and executes the SSC application on the CTEE.
%As there can be multiple SSC applications executing with temporal isolation inside a CTEE, this interface cleans up the memory spaces by default before loading the SSC onto memory.
%ii) \textit{NewData} interface facilitates the UAs that need to interact with the SSC application continuously.
%Whenever there is an input that FW does not understand it will be forwarded to the SSC application as NewData.
%SSC application contains the application logic to process this NewData and write corresponding output on the DRAM.
%iii) \textit{LdExecPreAtt} and iv)\textit{LdExecPostAtt} are two important interfaces provided by the FW to perform pre-execution and post-execution attestations respectively.
%As described in section~\ref{subsec:attest} pre-execution attestation include attestation over the \textit{chal}, Input, and SSC*.
%While post-execution attestation includes the Output from SSC along the \textit{chal}, Input, and SSC*.
%v)\textit{Clean} interface is the last interface provide by the FW to clean up the SSC memory regions after a SSC execution session on the CTEE.
%\begin{figure}[H]
%	\begin{centering}
%		\centering
%		\includegraphics[width=0.5\textwidth]{images/SSC_Firmware_memory_layout.pdf}
%		\caption{Memory Layout Of SSC}\label{fig: memory_ssc}
%	\end{centering}
%\end{figure}

%\begin{figure}[H]
%	\begin{centering}
%		\centering
%		\includegraphics[width=0.5\textwidth]{images/SSC_dumped_file_format.pdf}
%		\caption{Dumped File format of SSC bare-metal application}\label{fig:ssc_format}
%	\end{centering}
%\end{figure}

\subsection{Computational Applications}

Computational applications take input from the PS or other CTEEs, perform the intended computational operations, and send the outputs back.
They represent computational tasks, such as encryption, decryption, machine learning-based classification, etc., that do not need peripherals.
%\sysname protects such applications from code disclosure, memory corruption, and side channel attacks from the PS and other CTEEs.   
\emph{Example application:}
%Implement an AES algorithm running in there. Take input from DRAM. It supports 2 modes: 1) The key is encryption and decryption key is embedded in the application; 2) use an user supplied key.
We implement an AES accelerator SSA (SSA-1). %as an example for computational applications. %, which offers AES encryption and decryption services.
To use SSA-1, a UA places the plaintext or ciphertext in the SEB and notifies the SSA. 
When the encryption or decryption is finished, SSA-1 places the outputs on the SEB.

%takes input from shared DRAM or BRAM as input 
%We implement AES-CBC encryption and decryption as a SSC to run on a CTEE.
%The PS software executes this application to do the computational task securely, so the inputs, such as plaintext to encrypt or ciphertext to decrypt must come from the PS software.
%The UA puts these inputs in the shared DRAM SEB.
%One AES key is embedded in the application for the AES algorithm, but this application also facilitates user supplied keys for AES.
%The UA can define an arbitrary key in the shared DRAM SEB, indicate the SSC to carry out the AES encryption or decryption operation with its provided key. 
%Depending on the triggered operation (encryption or decryption), the SSC writes the outputs (ciphertext or plaintext) in the shared DRAM SEB. 

\subsection{Peripheral Interacting Applications}

Simple peripheral interacting applications control one or more peripherals, but they do not communicate with other SSAs or applications on the PS.
An example usage is cyber-physical applications that read from sensors, make local decisions, and control an actuator.
%\sysname protects such applications from attacks from compromised software running on PS or peripherals that are not connected to their CTEEs.
%Let us program this with button. Click a button show red. Click another button show yellow.
%Show the block diagram of this to show how the system and peripherals are isolated from other parts.
\emph{Example application:}
We develop an LED toggler SSA (SSA-2) that uses a button and an LED.
When the button is pressed, SSA-2 toggles the color of the LED.
Both the button and LED are directly connected to the CTEE of SSA-2 and cannot be accessed by the PS or other CTEEs.

\begin{comment}
\begin{lstlisting}[label={ssa2},caption={SSA-2 Code Snippet}, language=c] .
void GpioHandler(void *CallbackRef)
{
	XGpio *GpioPtr = (XGpio *)CallbackRef;
	IntrFlag = 1;
	XGpio_InterruptClear(GpioPtr, GlobalIntrMask);
}

int main()
{
	u32 *led = (u32 *)XPAR_RGB_PWM_0_PWM_AXI_BASEADDR;
	xil_printf("Wait for Button GPIO interrupt: \r\n");
	
	while(true) 
	{
		if(IntrFlag)
		{
			toggleLED(led);
		}
	}
	
	return 0;
}
\end{lstlisting}
Listing~\ref{ssa2} represents the code snippet of the LED Switch SSA, where it configures GpioHandler function as the button interrupt handler.
\end{comment}
%When the \firmware triggers the SSC execution, the button present in the device controls the LED light’s color.
%If we press the button on the device, the color of the LED becomes yellow, and if we do it again, the color changes to green, red, and so on.
%To provide physical isolation of these peripherals, we design the CTEE hardware in such a way so that only the CTEE executing the SSC has access to those two peripherals.
%The PS or other CTEEs running on the device are physically isolated from those peripherals. 
%
%Trusted Path with LED is a simple application to control the RGB value of a LED peripheral.
%Everything on the Zynq SoC is memory-mapped, the memory address of the LED peripheral is \verb|0x04A10000|.
%After booting the device, execution begins on the Cortex-A side, and the color of that LED peripheral is set to RED by default.
%When Cortex-A software triggers the Microblaze bare-metal application, it sets the color of the LED to blue for 1000 microseconds and displays a message through UART peripheral.
%This example application is converted to a \sysname SSC to demonstrate the process and usage of our system.
%The RGB value of the LED peripheral to blue here indicates the secure execution of the system.
%
%The untrusted app wants to execute SSC code, it loads the SSC file from SD card to shared memory(BRAM) with the CTEE.
%Then UA triggers the execution of the \firmware software module.
%The FW copies the SSC code to its  local memory after verifying the signature and hands over execution to the SSC.
%SSC executable starts the execution from a function called \verb|main| that the linker script puts at the beginning of the code section.
%
%%\begin{lstlisting}[ label={header},caption={Header file defining SSC #ifndef __LED_H_
%%#define __LED_H
%
%%oid main() __attribute__
%%((section (".ssc_entry")));
%
%%#endif
%%\end{lstlisting}
%
%A header file defines the entry point function for the SSC application with the attribute \verb|ssc_entry|.
%Listing~\ref{} is the header file for the Trusted Path with LED application, where we define the \verb|main| function as the entry point.
%
%\begin{lstlisting}[label={LED_C},caption={Function to change LED to blue}, language=c] 
%#include "LedHeader.h"
%
%BLUE =   {0x0000, 0x0000, 0x01ff};
%/*Defined with .ssc_entry attribute in Header*/
%void main()
%{
%    u32 *led = (u32*) LED_Address;
%    /*xil_printf invoked from Runtime*/
%    xil_printf("LED Blue from SSC");
%    /*xil_printf invoked from Runtime*/
%    setLED(led, BLUE);
%    return 0;
%}
%\end{lstlisting}
%
%In the definition of \verb|main| in a C file in Listing~\ref{LED_C}, it uses the local variable \verb|led| to denote the address of the RGB LED.
%Then it prints a string with \verb|xil_printf| Xilinx library function and calls a user-defined function \verb|setLED| to set the LED color.
%However, the \verb|xil_printf| function call will be redirected to the function from the \verb|runtime|, instead of having multiple copies of the same function.

\subsection{Peripheral and PS Interacting Applications}
\label{sec:DRM}

[Need to clearly explain why this app needs BYOT. Why TrustZone can;t provide the protection (code boot attack).]

Peripheral and PS interacting applications do not only control some peripherals but also continuously interacts with the UA.

\emph{Example application:}
We develop a music player SSA with digital rights management (SSA-3).
The untrusted module running on the PS takes user's commands, such as login (using username and Pin), logout, query (i.e., display a song's owner information), share (i.e., share a song to another user), play, pause, resume, and stop.
Depending on the user's request, it communicates with the SSA and forwards necessary data through SEB. 
 
%Table~\ref{tab:DRM_Audio_operations} lists the commands users can issue to the UA.
%The UA continuously interact with the SSA and handles user interaction task.
%The purpose of this application: is to ensure the DRM properties while continuously interacting with the UA, and ensure the confidentiality, integrity, authenticity of any communication data with the UA.

%\begin{comment}
%\begin{table}[h]
%\center
%\scriptsize
%\begin{tabular} {c|c}
%\hline
%Command           & Description \\ \hline\hline
%login & login with a username and pin \\ \hline           
%logout & logout current user \\ \hline     
%query\_song & retrieve the information of a song \\ \hline
%share & share a song with another user \\ \hline
%%digital\_out & Output the specified song content as a digital file \\ \hline         
%play & play a song \\ \hline                         
%pause & pause playing \\ \hline                         
%resume & resume playing\\ \hline      
%%restart & Play the current song from beginning \\ \hline            
%stop & stop playing \\ \hline                          
%\end{tabular}
%\caption{SSA-3 User Interface}
%\label{tab:DRM_Audio_operations}
%\end{table}
%\end{comment}
The trusted module is the SSA running on the CTEE, which implements the DRM properties of the music player.
Allow only authorized users to play songs, regional provisioning of songs, prevent unprovisioned media files from being played are some of the DRM properties that the SSA needs to ensure.
To validate those properties at runtime, the required DRM meta-information is embedded in the SSA or put onto the media files themselves.
For example, user passwords, encryption keys are embedded into the SSA, however, region lock, owner and shared user information, etc. are put onto the media files.
Embedded information is only available to the SSA as it is in BRAM of the CTEE, and the media files are authenticated and can only be decrypted by the SSA on BRAM.
So the untrusted module at runtime does not have access to sensitive data to temper with. 


%To prepare the media files at build time, we add meta-information to the audio files along with media data.
%The meta-information includes the owner of the song, shared users, lock, and regional permissions.
%In this example application, the media files will go through the UA before reaching the SSA.
%To prevent the UA from manipulating the file content, we add a signature and encrypt all data with a developer-defined symmetric key.
%We implant the symmetric key on the SSA, and encrypted SSA's are only decrypted by the \firmware in BRAM.
%Thus, the UA has no access to the symmetric key.
%
%Along with the boot files and SSAs, we also put the media files on the SD card.
%After the device boots, the UA has full access to the encrypted files.
%The UA provides several I/O functionalities of the music player to interact with the users.
%Table \ref{tab:DRM_Audio_operations} represents the allowed operation that a user can perform.
%The UA in turn communicates to the SSA with required data to carry out the operation through SEB.
%The data may vary for each operation: for example in login operation, the UA provides the user-provided user name and password in the SEB.
%The user passwords are embedded in the SSA and compared with user input at runtime.
%On the other hand, in play operation, the UA puts the constructed media file data from the SD card to the SEB.
%When the SSA receives the data from the SEB, it decrypts and verifies the signature.
%Then the SSA implements the logic to maintain DRM properties for the player.
%
%For some operations: such as share songs, the SSA needs to modify the meta-information in the media files.
%The SSA modifies the data, generates signatures, encrypts it, and hands over file content to UA through SEB.
%The UA then writes the content on the SD card file.
%So even if the UA is reading and writing file contents, it can only access the encrypted forms.
%Other SSA outputs such as query song operation output are put into the SEB for the UA to interact with the user.



\subsection{Intercommunicating SSA}
Intercommunicating SSAs represents a set of applications where multiple SSA runs on different physically separated CTEEs and needs secure intercommunication between them to carry out the interdependent sensitive task.
%Individual CTEEs execute their sensitive applications in isolation, and secure communication allows them to exchange sensitive data without going through the PS.

\emph{Example application:}
As an example, we develop two computational applications deployed in two physically separated CTEEs.
When the untrusted module wants to authenticate and decrypt some data, it sends the signature and ciphertext through the SEB to the CTEE-1's SSA.
%The SSA of CTEE-1 executes the sensitive task of data authentication and decryption.
The SSA of CTEE-1 performs the AES decryption task and internally utilizes the SSA on CTEE-2 to generate the signature (SHA512-HMAC).
The communication between the SSAs are through a shared BRAM without untrusted PS software access.
%Implementing through \sysname, these security-sensitive operations are hidden from the UA and keys from unprotected DRAM.
%CTEE-1 has a shared SEB to receive the signature and ciphertext from the  UA and the CTEE-2 receives its data from CTEE-1.
%A BRAM is shared between both CTEEs for secure communication, as the PS does not have access to the shared BRAM.
%Both CTEEs have their keys embedded in the SSAs.
This example also illustrates the dynamic and static loading of SSAs onto the CTEEs.
While the \firmware of the CTEE-1 dynamically loads the AES accelerator SSA into its BRAM, the SSA on CTEE-2 is loaded statically onto the BRAM with the bitstream.
%After the device boots, the PS software programs the PL side with bitstream containing the \firmware on CTEE-1 for dynamic loading of SSAs, and static authentication SSA on CTEE-2. 
%extend the previous application. The decryption part is running in one computational CTEE.
%The music playing is in another CTEE.
%Can they use BRAM to exchange message and plaintext music?

%\subsection{Peripheral, PS and CTEE Interacting Applications}
%\label{sec:DRM}
%
%Peripheral, PS, and CTEE interacting applications represent a set of applications where security-sensitive tasks are distributed into multiple modules and assigned to multiple CTEEs.
%Multiple CTEEs executing the different modules not only interact with the PS software but also interacts between themselves.
%Multiple CTEEs to execute different parts of the application achieves physical isolation among the hardware modules and speed up the execution. 
%
%As an example of this set of applications, we divide the previous Secure Digital Rights Management (DRM) application into two different logic modules.
%For secure 2-way inter-CTEE communication, we define the PL hardware design with a shared BRAM region between the CTEEs.
%We achieve the required synchronization between the executions of the different CTEEs by this shared BRAM region.
%This shared BRAM region is physically isolated from the untrusted PS side
%The encrypted audio files will be decrypted by one CTEE, and playing music application logic is carried out by the other CTEE.
%The CTEE performing the decryption operation will decrypt the ciphertext and write the plaintext on the shared BRAM region for the other CTEE.


